Surface detachment and bed entrainment of fluvial plastics

Over the last decade, fluvial plastics have been identified as major threat to aquatic environments and human health. In order to develop adequate mitigation strategies for plastic pollution, a fundamental process understanding of riverine plastic transport is of significant importance. In this context, the implementation of research findings into numerical simulation environments is anticipated to enhance modelling capabilities and to support a rigorous decision making. Recent experimental research has focused on the incipient motion of plastic particles, as well as on the effects of surface tension on plastic concentration profiles. While these investigations have advanced the state-of-the-art knowledge, current literature still displays a lack of basic insights into layer-specific plastic transport physics. In this study, first principles are applied to advance knowledge on free-surface detachment and bed entrainment of fluvial plastics. A novel relationship for the critical surface detachment velocity is derived, followed by the development of a framework that allows to relate plastic Shields parameters to those of natural sediments. Overall, it is anticipated that these developments will trigger new research within the plastics community, and it is hoped that present findings will be implemented into Lagrangian particle tracking software.

==> Figures/FigA1.tex <==
\begin{tikzpicture}

\node at (-6,0)
{\includegraphics{Figures/FigA1.pdf}};

\node[align=center,color=black] at(-8,2.5) {(\textit{a})};

\node[align=center,color=black] at(-3,2.5) {(\textit{b})};

\node at (-3,-3) {

\begin{groupplot}[
     group style = {group size = 2 by 1,horizontal sep=2 cm,vertical sep=1.8cm}]
     
\nextgroupplot[height = 6 cm,
     width =8 cm,
     xlabel={$D_p$ (mm)},
     ylabel={$\left(h_w/D_p\right)_\text{cr}$}, 
     grid=both,
     xmin=0,
     xmax=30,
     ymin=0,
    ymax=1, 
  domain=0.01:1000,samples=400,
   legend style={cells={align=left},anchor = south west,at={(0,1.1)},font=\normalsize},  ]

  
\addplot+[densely dashed,color=black,mark=none,line width=2] 
table{		
0.0100000000000000	0.500000000000000
0.110000000000000	0.500000000000000
0.210000000000000	0.500000000000000
0.310000000000000	0.501000000000000
0.410000000000000	0.501000000000000
0.510000000000000	0.502000000000000
0.610000000000000	0.503000000000000
0.710000000000000	0.504000000000000
0.810000000000000	0.506000000000000
0.910000000000000	0.507000000000000
1.01000000000000	0.509000000000000
1.11000000000000	0.511000000000000
1.21000000000000	0.513000000000000
1.31000000000000	0.515000000000000
1.41000000000000	0.517000000000000
1.51000000000000	0.520000000000000
1.61000000000000	0.523000000000000
1.71000000000000	0.526000000000000
1.81000000000000	0.529000000000000
1.91000000000000	0.532000000000000
2.01000000000000	0.535000000000000
2.11000000000000	0.539000000000000
2.21000000000000	0.543000000000000
2.31000000000000	0.546000000000000
2.41000000000000	0.550000000000000
2.51000000000000	0.555000000000000
2.61000000000000	0.559000000000000
2.71000000000000	0.563000000000000
2.81000000000000	0.568000000000000
2.91000000000000	0.572000000000000
3.01000000000000	0.577000000000000
3.11000000000000	0.582000000000000
3.21000000000000	0.587000000000000
3.31000000000000	0.592000000000000
3.41000000000000	0.597000000000000
3.51000000000000	0.602000000000000
3.61000000000000	0.607000000000000
3.71000000000000	0.612000000000000
3.81000000000000	0.618000000000000
3.91000000000000	0.623000000000000
4.01000000000000	0.628000000000000
4.11000000000000	0.633000000000000
4.21000000000000	0.639000000000000
4.31000000000000	0.644000000000000
4.41000000000000	0.649000000000000
4.51000000000000	0.654000000000000
4.61000000000000	0.660000000000000
4.71000000000000	0.665000000000000
4.81000000000000	0.670000000000000
4.91000000000000	0.675000000000000
5.01000000000000	0.680000000000000
5.11000000000000	0.685000000000000
5.21000000000000	0.690000000000000
5.31000000000000	0.694000000000000
5.41000000000000	0.699000000000000
5.51000000000000	0.704000000000000
5.61000000000000	0.708000000000000
5.71000000000000	0.713000000000000
5.81000000000000	0.717000000000000
5.91000000000000	0.722000000000000
6.01000000000000	0.726000000000000
6.11000000000000	0.730000000000000
6.21000000000000	0.734000000000000
6.31000000000000	0.738000000000000
6.41000000000000	0.742000000000000
6.51000000000000	0.746000000000000
6.61000000000000	0.750000000000000
6.71000000000000	0.754000000000000
6.81000000000000	0.758000000000000
6.91000000000000	0.761000000000000
7.01000000000000	0.765000000000000
7.11000000000000	0.768000000000000
7.21000000000000	0.771000000000000
7.31000000000000	0.775000000000000
7.41000000000000	0.778000000000000
7.51000000000000	0.781000000000000
7.61000000000000	0.784000000000000
7.71000000000000	0.787000000000000
7.81000000000000	0.790000000000000
7.91000000000000	0.793000000000000
8.01000000000000	0.796000000000000
8.11000000000000	0.799000000000000
8.21000000000000	0.802000000000000
8.31000000000000	0.804000000000000
8.41000000000000	0.807000000000000
8.51000000000000	0.809000000000000
8.61000000000000	0.812000000000000
8.71000000000000	0.814000000000000
8.81000000000000	0.817000000000000
8.91000000000000	0.819000000000000
9.01000000000000	0.821000000000000
9.11000000000000	0.824000000000000
9.21000000000000	0.826000000000000
9.31000000000000	0.828000000000000
9.41000000000000	0.830000000000000
9.51000000000000	0.832000000000000
9.61000000000000	0.834000000000000
9.71000000000000	0.836000000000000
9.81000000000000	0.838000000000000
9.91000000000000	0.840000000000000
10.0100000000000	0.842000000000000
10.1100000000000	0.844000000000000
10.2100000000000	0.846000000000000
10.3100000000000	0.848000000000000
10.4100000000000	0.849000000000000
10.5100000000000	0.851000000000000
10.6100000000000	0.853000000000000
10.7100000000000	0.855000000000000
10.8100000000000	0.856000000000000
10.9100000000000	0.858000000000000
11.0100000000000	0.859000000000000
11.1100000000000	0.861000000000000
11.2100000000000	0.862000000000000
11.3100000000000	0.864000000000000
11.4100000000000	0.865000000000000
11.5100000000000	0.867000000000000
11.6100000000000	0.868000000000000
11.7100000000000	0.870000000000000
11.8100000000000	0.871000000000000
11.9100000000000	0.872000000000000
12.0100000000000	0.874000000000000
12.1100000000000	0.875000000000000
12.2100000000000	0.876000000000000
12.3100000000000	0.877000000000000
12.4100000000000	0.879000000000000
12.5100000000000	0.880000000000000
12.6100000000000	0.881000000000000
12.7100000000000	0.882000000000000
12.8100000000000	0.883000000000000
12.9100000000000	0.884000000000000
13.0100000000000	0.885000000000000
13.1100000000000	0.887000000000000
13.2100000000000	0.888000000000000
13.3100000000000	0.889000000000000
13.4100000000000	0.890000000000000
13.5100000000000	0.891000000000000
13.6100000000000	0.892000000000000
13.7100000000000	0.893000000000000
13.8100000000000	0.894000000000000
13.9100000000000	0.895000000000000
14.0100000000000	0.896000000000000
14.1100000000000	0.897000000000000
14.2100000000000	0.897000000000000
14.3100000000000	0.898000000000000
14.4100000000000	0.899000000000000
14.5100000000000	0.900000000000000
14.6100000000000	0.901000000000000
14.7100000000000	0.902000000000000
14.8100000000000	0.903000000000000
14.9100000000000	0.904000000000000
15.0100000000000	0.904000000000000
15.1100000000000	0.905000000000000
15.2100000000000	0.906000000000000
15.3100000000000	0.907000000000000
15.4100000000000	0.907000000000000
15.5100000000000	0.908000000000000
15.6100000000000	0.909000000000000
15.7100000000000	0.910000000000000
15.8100000000000	0.910000000000000
15.9100000000000	0.911000000000000
16.0100000000000	0.912000000000000
16.1100000000000	0.913000000000000
16.2100000000000	0.913000000000000
16.3100000000000	0.914000000000000
16.4100000000000	0.915000000000000
16.5100000000000	0.915000000000000
16.6100000000000	0.916000000000000
16.7100000000000	0.917000000000000
16.8100000000000	0.917000000000000
16.9100000000000	0.918000000000000
17.0100000000000	0.918000000000000
17.1100000000000	0.919000000000000
17.2100000000000	0.920000000000000
17.3100000000000	0.920000000000000
17.4100000000000	0.921000000000000
17.5100000000000	0.921000000000000
17.6100000000000	0.922000000000000
17.7100000000000	0.923000000000000
17.8100000000000	0.923000000000000
17.9100000000000	0.924000000000000
18.0100000000000	0.924000000000000
18.1100000000000	0.925000000000000
18.2100000000000	0.925000000000000
18.3100000000000	0.926000000000000
18.4100000000000	0.926000000000000
18.5100000000000	0.927000000000000
18.6100000000000	0.927000000000000
18.7100000000000	0.928000000000000
18.8100000000000	0.928000000000000
18.9100000000000	0.929000000000000
19.0100000000000	0.929000000000000
19.1100000000000	0.930000000000000
19.2100000000000	0.930000000000000
19.3100000000000	0.931000000000000
19.4100000000000	0.931000000000000
19.5100000000000	0.932000000000000
19.6100000000000	0.932000000000000
19.7100000000000	0.933000000000000
19.8100000000000	0.933000000000000
19.9100000000000	0.933000000000000
20.0100000000000	0.934000000000000
20.1100000000000	0.934000000000000
20.2100000000000	0.935000000000000
20.3100000000000	0.935000000000000
20.4100000000000	0.935000000000000
20.5100000000000	0.936000000000000
20.6100000000000	0.936000000000000
20.7100000000000	0.937000000000000
20.8100000000000	0.937000000000000
20.9100000000000	0.937000000000000
21.0100000000000	0.938000000000000
21.1100000000000	0.938000000000000
21.2100000000000	0.939000000000000
21.3100000000000	0.939000000000000
21.4100000000000	0.939000000000000
21.5100000000000	0.940000000000000
21.6100000000000	0.940000000000000
21.7100000000000	0.940000000000000
21.8100000000000	0.941000000000000
21.9100000000000	0.941000000000000
22.0100000000000	0.942000000000000
22.1100000000000	0.942000000000000
22.2100000000000	0.942000000000000
22.3100000000000	0.943000000000000
22.4100000000000	0.943000000000000
22.5100000000000	0.943000000000000
22.6100000000000	0.944000000000000
22.7100000000000	0.944000000000000
22.8100000000000	0.944000000000000
22.9100000000000	0.944000000000000
23.0100000000000	0.945000000000000
23.1100000000000	0.945000000000000
23.2100000000000	0.945000000000000
23.3100000000000	0.946000000000000
23.4100000000000	0.946000000000000
23.5100000000000	0.946000000000000
23.6100000000000	0.947000000000000
23.7100000000000	0.947000000000000
23.8100000000000	0.947000000000000
23.9100000000000	0.947000000000000
24.0100000000000	0.948000000000000
24.1100000000000	0.948000000000000
24.2100000000000	0.948000000000000
24.3100000000000	0.949000000000000
24.4100000000000	0.949000000000000
24.5100000000000	0.949000000000000
24.6100000000000	0.949000000000000
24.7100000000000	0.950000000000000
24.8100000000000	0.950000000000000
24.9100000000000	0.950000000000000
25.0100000000000	0.950000000000000
25.1100000000000	0.951000000000000
25.2100000000000	0.951000000000000
25.3100000000000	0.951000000000000
25.4100000000000	0.951000000000000
25.5100000000000	0.952000000000000
25.6100000000000	0.952000000000000
25.7100000000000	0.952000000000000
25.8100000000000	0.952000000000000
25.9100000000000	0.953000000000000
26.0100000000000	0.953000000000000
26.1100000000000	0.953000000000000
26.2100000000000	0.953000000000000
26.3100000000000	0.954000000000000
26.4100000000000	0.954000000000000
26.5100000000000	0.954000000000000
26.6100000000000	0.954000000000000
26.7100000000000	0.955000000000000
26.8100000000000	0.955000000000000
26.9100000000000	0.955000000000000
27.0100000000000	0.955000000000000
27.1100000000000	0.955000000000000
27.2100000000000	0.956000000000000
27.3100000000000	0.956000000000000
27.4100000000000	0.956000000000000
27.5100000000000	0.956000000000000
27.6100000000000	0.956000000000000
27.7100000000000	0.957000000000000
27.8100000000000	0.957000000000000
27.9100000000000	0.957000000000000
28.0100000000000	0.957000000000000
28.1100000000000	0.957000000000000
28.2100000000000	0.958000000000000
28.3100000000000	0.958000000000000
28.4100000000000	0.958000000000000
28.5100000000000	0.958000000000000
28.6100000000000	0.958000000000000
28.7100000000000	0.959000000000000
28.8100000000000	0.959000000000000
28.9100000000000	0.959000000000000
29.0100000000000	0.959000000000000
29.1100000000000	0.959000000000000
29.2100000000000	0.960000000000000
29.3100000000000	0.960000000000000
29.4100000000000	0.960000000000000
29.5100000000000	0.960000000000000
29.6100000000000	0.960000000000000
29.7100000000000	0.960000000000000
29.8100000000000	0.961000000000000
29.9100000000000	0.961000000000000
};


\end{groupplot}
};



\end{tikzpicture}

  

==> Figures/fig4.tex <==
\pgfplotstableread{
Re theta
0.0439504950495076	0.121406916494082
0.0505066758615054	0.121308490942955
0.0580427597073256	0.121195282452036
0.0666991296295381	0.121065151127494
0.0766497263569791	0.120915441991814
0.0880642740950892	0.120743550196060
0.101166322325205	0.120546043995473
0.116194979120544	0.120319236000934
0.133463427143130	0.120058294400352
0.153246227629292	0.119758939161087
0.175944254834040	0.119414942409864
0.201969732451309	0.119019858281995
0.231760420546636	0.118566805223917
0.265904871702721	0.118046555739517
0.304941325044775	0.117450596356257
0.349581712313719	0.116767723488841
0.400598367828266	0.115985788442975
0.458769608479605	0.115092580944408
0.525162907514406	0.114071558821337
0.600721570834082	0.112908323948528
0.686594582071820	0.111585755364224
0.784060949879249	0.110085465616022
0.894542862693508	0.108388029954893
1.01936758707595	0.106477231758176
1.16021396570149	0.104333993079803
1.31853090355694	0.101946239002979
1.49613414768481	0.0993010053364325
1.69485910664836	0.0963911474453624
1.91623716510733	0.0932213840831835
2.16231962702673	0.0897977255054759
2.43494456380376	0.0861393846677414
2.73610249741867	0.0822744277739670
3.06759114649268	0.0782444689328921
3.43216377847556	0.0740906699772513
3.83187749566039	0.0698729629220146
4.27022795974784	0.0656451966858493
4.75086220904907	0.0614693298225417
5.27843658735360	0.0574062431184857
5.85896982068522	0.0535138448103208
6.50103767034144	0.0498418257855202
7.21424818451697	0.0464433455391226
8.01371402109567	0.0433552780330927
8.91724934852883	0.0406173270853672
9.94999764860834	0.0382579148443920
11.1426909220162	0.0363024545792351
12.5365593153802	0.0347627739044170
14.1785232131302	0.0336406116934789
16.1250653901696	0.0329165232155409
18.4360954426186	0.0325509839170182
21.1758541781849	0.0324858088122925
24.4094470400022	0.0326533505237665
28.2088894514462	0.0329871217733632
32.6508591901528	0.0334296108941300
37.8238520345640	0.0339359803320998
43.8336336873920	0.0344740652509392
50.7977903194842	0.0350214362806513
58.8555167932795	0.0355635496120611
68.1706896355707	0.0360913915100739
78.9327639997515	0.0365995375035718
91.3538515795328	0.0370847059809147
105.685995862488	0.0375455227154792
122.218650493523	0.0379815545291273
141.284071432924	0.0383929718603901
163.259986358716	0.0387802730279231
188.593978601210	0.0391444167515172
217.780883816095	0.0394862175585878
251.413267644171	0.0398068524505028
290.159075103524	0.0401073631223815
334.778820820178	0.0403887654034721
386.173348259451	0.0406522180327317
445.354052658195	0.0408987062852178
513.494195305911	0.0411292361639576
591.940793515431	0.0413447643535780
682.248501870532	0.0415462171231836
786.193141283134	0.0417344505484713
905.842855949289	0.0419103191084451
1043.54091172341	0.0420745788675542
1202.01074665509	0.0422279814616775
1384.36701886509	0.0423712169574755
1594.19838191165	0.0425049419988141
1835.64075877569	0.0426297779835233
2113.42486856748	0.0427462964125952
2433.01695284250	0.0428550455657773
2800.69331130927	0.0429565351415016
3223.68188499542	0.0430512449791758
3710.25386688230	0.0431396167078527
4269.98323465232	0.0432220751421415
4913.80144233010	0.0432990066073146
5654.38543876921	0.0433707847770636
6506.18267854640	0.0434377464441257
7485.92832078969	0.0435002165161935
8612.74844665624	0.0435584911129715
9908.78394867454	0.0436128543144869
11399.3529771746	0.0436635651214936
13113.5594360787	0.0437108663789080
15085.0616616987	0.0437549896177154
17352.2950684499	0.0437961449764514
19959.6633342992	0.0438345328155473
22958.1439594208	0.0438703386295664
26406.4356435428	0.0439037363267262
}\Shields

\begin{tikzpicture}
\begin{groupplot}[
     group style = {group size = 1 by 2,horizontal sep=2.5cm,vertical sep=1.8cm}]



\nextgroupplot[height = 6cm,
     width =12 cm,
     ylabel={$\theta_{\text{cr},s}$, $\theta_{\text{cr},p}$},
     xlabel={$Re_{*}$},
     grid=both,
     xmin=0.1,
     xmax=1000,
     ymin=0.001,
    ymax=1, 
    xmode=log,
    ymode=log,
    legend columns=2,
%transpose legend,
  domain=0.01:1000,samples=400,
   legend style={cells={align=left},anchor = south west,at={(0,1.1)},font=\small},  ]


\addplot [fill=red,color=red,mark=*,only marks,fill opacity=0.5,draw opacity=0.8, mark size=2.5,draw= black,clip mode=individual]
table[row sep=crcr]{%	
1000 1000	\\
};\addlegendentry{\citeA{Waldschlaeger2019} \, }

\draw [black, draw opacity=0, name path=A] plot [smooth, tension=0] coordinates {(0.01,0.001) (5,0.001)};
\draw [black, draw opacity=0, name path=B] plot [smooth, tension=0] coordinates {(0.01,100) (5,100)};
\addplot+[teal!50!black, opacity=0.1] fill between[of=A and B]; \addlegendentry{hydraulically smooth } %($Re_{*,s} < \approx 5$)}



\addplot [fill=black,color=black,mark=diamond*,only marks,fill opacity=0.5,draw opacity=0.8, mark size=3,draw= black,clip mode=individual]
table[row sep=crcr]{%
1000 1000	\\
};\addlegendentry{\citeA{Goral2023}}



\draw [black, draw opacity=0, name path=A] plot [smooth, tension=0] coordinates {(5,0.001) (70,0.001)};
\draw [black, draw opacity=0, name path=B] plot [smooth, tension=0] coordinates {(5,100) (70,100)};
\addplot+[violet, opacity=0.1] fill between[of=A and B]; \addlegendentry{transitionally rough } %($\approx 5 < Re_{*,s} < \approx 70$)}

%\addplot [color=red,mark=none,line width=2]  table [x=Re, y=theta] {\Shields};

\addplot+[densely dashed,color=black,mark=none,line width=2] {0.165*(x+0.6)^(-0.8)+0.045*exp(-40*x^(-1.3))}; \addlegendentry{Eq. (\ref{eqSui})}

\draw [black, draw opacity=0, name path=A] plot [smooth, tension=0] coordinates {(70,0.001) (1000,0.001)};
\draw [black, draw opacity=0, name path=B] plot [smooth, tension=0] coordinates {(70,100) (1000,100)};
\addplot+[orange, opacity=0.1] fill between[of=A and B]; \addlegendentry{hydraulically rough } % ($Re_{*,s} > \approx 70$)}


 
%\node[align=center,fill=white,fill opacity=0.3,text opacity=1] at (rel axis cs:0.1,0.9) {(\textit{b})};  

\node[align=center,fill=white,fill opacity=0.6,text opacity=1] at (rel axis cs:0.5,0.15) {no motion};  

\node[align=center,fill=white,fill opacity=0.6,text opacity=1] at (rel axis cs:0.5,0.8) {motion};  
  



\addplot [fill=red,color=red,mark=*,only marks,fill opacity=0.5,draw opacity=0.8, mark size=2.5,draw= black,clip mode=individual]
table[row sep=crcr]{%
1.382961272	0.04044302	\\
3.525200832	0.055406937	\\
15.88901533	0.120115769	\\
6.852864562	0.091805655	\\
1.080127283	0.005597394	\\
2.625610959	0.006973802	\\
12.09157803	0.015782815	\\
5.304307272	0.012479435	\\
1.860584102	0.013855445	\\
5.336891878	0.024036517	\\
30.80000994	0.085429151	\\
11.57835132	0.049604023	\\
1.716209805	0.023533192	\\
4.893567056	0.040342616	\\
25.38360858	0.115832207	\\
10.18071038	0.076559282	\\
1.931200317	0.013998363	\\
5.446248542	0.023474178	\\
25.43379039	0.05462951	\\
8.110969719	0.0228281	\\
24.56676286	0.067957866	\\
9.039778056	0.037807545	\\
2.14247439	0.017228755	\\
5.682619527	0.025555986	\\
22.03113205	0.040990079	\\
8.49712356	0.025053481	\\
4.043831731	0.009972261	\\
9.466774944	0.011523502	\\
42.19983696	0.024434955	\\
16.7366507	0.015792329	\\
4.311646538	0.009818031	\\
9.557368156	0.010171561	\\
39.66632526	0.018696683	\\
17.76791577	0.015413905	\\
3.536705458	0.017122994	\\
31.57677448	0.030711426	\\
12.99284625	0.02136447	\\
3.237429335	0.005723264	\\
8.081460016	0.007519617	\\
44.49421035	0.024323874	\\
16.10675261	0.013096667	\\
2.923908515	0.009773863	\\
31.07477015	0.024839169	\\
12.0597105	0.015371422	\\
2.936961743	0.010170521	\\
34.57095842	0.031706769	\\
16.66232027	0.030263502	\\
3.210734547	0.007459151	\\
8.411450271	0.010794319	\\
40.53542085	0.026750537	\\
14.81552044	0.014683042	\\
6.584696744	0.03108565	\\
22.02517053	0.033673346	\\
138.7410324	0.046577054	\\
43.39379527	0.037948627	\\
};


\addplot [fill=black,color=black,mark=diamond*,only marks,fill opacity=0.5,draw opacity=0.8, mark size=3,draw= black,clip mode=individual]
table[row sep=crcr]{%
1.1158	0.0117	\\
1.1321	0.0060	\\
1.4994	0.0071	\\
0.5786	0.0056	\\
1.6944	0.0068	\\
1.7591	0.0057	\\
1.1122	0.0086	\\
1.0589	0.0061	\\
1.1571	0.0066	\\
1.2165	0.0065	\\
1.2344	0.0068	\\
1.2363	0.0064	\\
1.3313	0.0067	\\
1.3627	0.0064	\\
1.4230	0.0060	\\
1.5849	0.0142	\\
1.7396	0.0133	\\
1.5660	0.0105	\\
1.8579	0.0201	\\
1.9424	0.0193	\\
1.8898	0.0130	\\
1.8852	0.0118	\\
1.7887	0.0096	\\
2.0313	0.0229	\\
1.9035	0.0167	\\
1.9157	0.0131	\\
1.1900	0.0097	\\
1.3414	0.0080	\\
1.4175	0.0082	\\
1.2412	0.0082	\\
1.4511	0.0073	\\
1.5629	0.0071	\\
1.2886	0.0087	\\
1.2377	0.0105	\\
1.1717	0.0146	\\
1.1038	0.0106	\\
1.2733	0.0125	\\
1.3075	0.0128	\\
1.2379	0.0090	\\
1.4532	0.0109	\\
1.4085	0.0093	\\
1.4691	0.0092	\\
1.5815	0.0091	\\
1.6286	0.0080	\\
1.4421	0.0151	\\
1.6580	0.0173	\\
1.6724	0.0161	\\
1.7193	0.0133	\\
1.7314	0.0125	\\
1.7527	0.0103	\\
1.2929	0.0155	\\
1.3288	0.0130	\\
1.2820	0.0099	\\
0.8577	0.0170	\\
0.8807	0.0143	\\
1.0269	0.0306	\\
0.9488	0.0208	\\
0.5781	0.0130	\\
0.6003	0.0081	\\
1.2421	0.0100	\\
1.7421	0.0099	\\
2.0714	0.0075	\\
1.7334	0.0105	\\
1.0703	0.0081	\\
};



\end{groupplot}
\end{tikzpicture}

==> Figures/fig5.tex <==
\begin{tikzpicture}
\begin{groupplot}[
     group style = {group size = 2 by 1,horizontal sep=1.5 cm,vertical sep=1.8cm}]


\nextgroupplot[height = 6 cm,
     width =6 cm,
     ylabel={$\frac{\theta_{\text{cr},p}}{ \theta_{\text{cr},s}} \frac{\beta_p}{\beta_s}  \frac{\tan{(\phi_s)}}{\tan{(\phi_p)}} $},
     xlabel={$D_p/D_s$},
     grid=both,
     xmin=0.01,
     xmax=100,
     ymin=0.05,
    ymax=15, 
    xmode=log,
    ymode=log,
    legend columns=2,
    legend cell align={left},
%transpose legend,
  domain=0.01:1000,samples=400,
   legend style={cells={align=left},anchor = south west,at={(0,1.2)},font=\normalsize}]

\node[align=center,fill=white,fill opacity=0.3,text opacity=1] at (rel axis cs:0.1,0.1) {(\textit{a})};  

\addplot [fill=red,color=red,mark=*,only marks,fill opacity=0.5,draw opacity=0.8, mark size=2.5,draw= black,clip mode=individual]
table[row sep=crcr]{%	
1000 1000	\\
};\addlegendentry{\citeA{Waldschlaeger2019} \, \, \\
($\tan{(\phi_p)}/ \tan{(\phi_s)} = 0.5588$)}


\addplot+[densely dotted,color=black,mark=none,line width=1.5] 
table[row sep=crcr]{%
1000 1000	\\
}; \addlegendentry{1:1}

\addplot [fill=black,color=black,mark=diamond*,only marks,fill opacity=0.5,draw opacity=0.8, mark size=3,draw= black,clip mode=individual]
table[row sep=crcr]{%
1000 1000	\\
};\addlegendentry{\citeA{Goral2023} \\ ($\tan{(\phi_p)}/ \tan{(\phi_s)} = 0.55$)}

\addplot+[densely dotted,color=violet,mark=none,line width=1] 
table[row sep=crcr]{%
1000 1000	\\
}; \addlegendentry{$\pm 20 \%$}

\addplot+[mark=none,color=black,line width=1.5] {x^(-0.6)}; \addlegendentry{$\left(D_p/D_s\right)^{c_2}$ with $c_2 = -0.6$}

\addplot+[densely dashed,color=black,mark=none,line width=2] 
table[row sep=crcr]{%
1000 1000	\\
}; \addlegendentry{Eq. (\ref{eqSui})}



\addplot [fill=red,color=red,mark=*,only marks,fill opacity=0.5,draw opacity=0.8, mark size=2.5,draw= black,clip mode=individual]
table{%	
10.73	0.04773598
4.93	0.072417744
1.61	1.377392087
3.26	0.264695548
1.00	1.567210312
1.00	1.695027276
1.00	1.839211183
1.00	1.639715531
5.82	0.811392335
2.67	1.996648594
0.87	7.067375328
1.77	5.052603898
2.54	0.355505545
1.17	1.005239555
0.38	1.751278998
0.77	1.189817658
6.76	0.163012892
3.10	0.371082366
1.01	0.937646026
2.05	0.643038719
5.29	0.265741338
2.43	0.678413513
0.79	1.316995584
1.61	0.924589817
2.76	0.21276827
1.27	0.706249227
0.41	1.763082435
0.84	0.839522348
0.31	2.213477767
0.63	1.431679807
5.51	0.420530364
2.53	0.752447922
0.83	1.208926749
1.68	0.977260044
5.51	0.499481005
2.53	0.768035369
0.83	1.079510162
1.68	1.084112524
3.47	0.465946322
0.52	1.136693352
1.06	0.985642549
3.47	0.234025105
0.52	0.922674392
1.06	0.715154192
5.48	0.152982895
2.52	0.530469652
0.82	1.954318449
1.67	1.422246061
3.45	0.196862699
1.59	0.669003138
0.52	2.209997266
1.05	1.742508404
5.48	0.150114386
0.82	0.707380094
1.67	0.814826914
};

\addplot [fill=black,color=black,mark=diamond*,only marks,fill opacity=0.5,draw opacity=0.8, mark size=3,draw= black,clip mode=individual]
table{%
5.56	0.19827359
11.11	0.102825006
16.67	0.140650101
17.22	0.070639809
22.22	0.144622254
27.78	0.125391429
14.56	0.16193163
16.02	0.122369598
17.26	0.150887309
19.08	0.112628571
21.00	0.129855695
22.62	0.133050493
25.44	0.12111641
27.40	0.125918468
31.80	0.113129153
14.56	0.247474126
16.02	0.222609305
21.00	0.189567574
6.85	0.205422242
10.87	0.254365233
17.26	0.212752657
22.62	0.221620399
27.40	0.190544551
16.88	0.141227051
22.51	0.120309602
28.14	0.089763148
5.40	0.253717928
6.80	0.214974306
2.34	0.99605985
2.95	0.648943022
16.00	0.210522192
20.15	0.185671947
25.39	0.184169761
8.68	0.264095048
9.94	0.213377329
10.94	0.297987771
11.79	0.333951643
15.78	0.153311779
17.37	0.221935006
18.71	0.201934279
22.76	0.165782833
24.52	0.183053765
29.70	0.14883013
12.53	0.147206753
13.79	0.151488402
14.85	0.121640636
19.88	0.171249273
21.42	0.139511342
26.98	0.146117618
13.79	0.140133732
20.68	0.124153199
24.12	0.130313692
24.12	0.121064633
27.57	0.117967035
34.46	0.119134709
34.46	0.132515527
34.46	0.156385954
};

\nextgroupplot[height = 6 cm,
     width =6 cm,
     ylabel={$\left(\theta_{\text{cr},p}\right)_{\text{calc}}$ [Eq. (\ref{eq13})]},
     xlabel={$\left(\theta_{\text{cr},p}\right)_{\text{meas}}$},
     grid=both,
     xmin=0.0,
     xmax=0.06,
     ymin=0,
    ymax=0.06, 
    legend columns=1,
    legend cell align={left},
%transpose legend,
  domain=0.01:1000,samples=400,
   legend style={cells={align=left},anchor = south west,at={(0,1.12)},font=\normalsize}]

\node[align=center,fill=white,fill opacity=0.3,text opacity=1] at (rel axis cs:0.1,0.9) {(\textit{b})};  

\addplot+[densely dotted,color=black,mark=none,line width=1.5] 
table[row sep=crcr]{%
0 0	\\
1 1	\\
};

\addplot+[densely dotted,color=violet,mark=none,line width=1] 
table[row sep=crcr]{%
0 0	\\
1 1.2\\
};

\addplot+[densely dotted,color=violet,mark=none,line width=1] 
table[row sep=crcr]{%
0 0	\\
1 0.8\\
};

\addplot [fill=red,color=red,mark=*,only marks,fill opacity=0.5,draw opacity=0.8, mark size=2.5,draw= black,clip mode=individual]
table{%
0.0033	0.0167
0.0033	0.0175
0.0248	0.0135
0.0072	0.0133
0.0311	0.0198
0.0337	0.0199
0.0466	0.0253
0.0379	0.0231
0.0389	0.0167
0.0533	0.0148
0.1155	0.0177
0.0883	0.0124
0.0151	0.0242
0.0223	0.0202
0.0358	0.0364
0.0219	0.0215
0.0050	0.0097
0.0065	0.0089
0.0211	0.0223
0.0114	0.0115
0.0062	0.0086
0.0090	0.0078
0.0224	0.0195
0.0123	0.0100
0.0113	0.0289
0.0189	0.0233
0.0440	0.0424
0.0184	0.0244
0.0548	0.0499
0.0305	0.0281
0.0114	0.0097
0.0131	0.0100
0.0279	0.0258
0.0180	0.0135
0.0129	0.0093
0.0134	0.0100
0.0246	0.0255
0.0203	0.0137
0.0138	0.0140
0.0248	0.0322
0.0172	0.0169
0.0079	0.0159
0.0200	0.0321
0.0124	0.0168
0.0069	0.0162
0.0119	0.0129
0.0423	0.0244
0.0246	0.0127
0.0093	0.0224
0.0159	0.0180
0.0456	0.0306
0.0302	0.0168
0.0050	0.0121
0.0157	0.0250
0.0150	0.0135
};

\addplot [fill=black,color=black,mark=diamond*,only marks,fill opacity=0.5,draw opacity=0.8, mark size=3,draw= black,clip mode=individual]
table{%
0.0117	0.0211
0.0060	0.0138
0.0071	0.0093
0.0056	0.0144
0.0068	0.0073
0.0057	0.0062
0.0086	0.0106
0.0061	0.0094
0.0066	0.0079
0.0065	0.0099
0.0068	0.0084
0.0064	0.0075
0.0067	0.0079
0.0064	0.0069
0.0060	0.0067
0.0162	0.0131
0.0167	0.0142
0.0116	0.0098
0.0434	0.0665
0.0329	0.0309
0.0176	0.0150
0.0140	0.0098
0.0103	0.0074
0.0093	0.0121
0.0078	0.0100
0.0059	0.0089
0.0170	0.0244
0.0143	0.0210
0.0612	0.0369
0.0415	0.0334
0.0229	0.0207
0.0167	0.0149
0.0131	0.0102
0.0146	0.0151
0.0106	0.0125
0.0125	0.0100
0.0128	0.0087
0.0090	0.0113
0.0109	0.0088
0.0093	0.0080
0.0092	0.0085
0.0091	0.0073
0.0080	0.0070
0.0151	0.0225
0.0173	0.0237
0.0161	0.0262
0.0133	0.0129
0.0125	0.0143
0.0103	0.0098
0.0097	0.0143
0.0080	0.0105
0.0082	0.0093
0.0082	0.0100
0.0073	0.0084
0.0071	0.0071
0.0087	0.0079
0.0105	0.0081
};


\end{groupplot}
\end{tikzpicture}

\vspace{0.3cm}

\begin{tikzpicture}
\begin{groupplot}[
     group style = {group size = 1 by 1,horizontal sep=2.5cm,vertical sep=1.8cm}]
     
\nextgroupplot[height = 6 cm,
     width =12cm,
     ylabel={$\theta_{\text{cr},s} = \theta_{\text{cr},p} / \left( \frac{\beta_s}{\beta_p}
     \frac{\tan{(\phi_p)}}{\tan{(\phi_s)}}  \left(\frac{D_p}{d_{50}}    \right)^{c_2} \right) $},
     xlabel={$Re_*$}, 
     grid=both,
     xmin=0.1,
     xmax=1000,
     ymin=0.001,
    ymax=5, 
    xmode=log,
    ymode=log,
    legend columns=2,
%transpose legend,
  domain=0.01:1000,samples=400,
   legend style={cells={align=left},anchor = south west,at={(0,1.1)},font=\normalsize},  ]




\node[align=center,fill=white,fill opacity=0.3,text opacity=1] at (rel axis cs:0.04,0.9) {(\textit{c})}; 

\node[align=center,fill=white,fill opacity=0.6,text opacity=1] at (rel axis cs:0.5,0.2) {no motion};  

\node[align=center,fill=white,fill opacity=0.6,text opacity=1] at (rel axis cs:0.5,0.8) {motion};  
  
\addplot+[densely dashed,color=black,mark=none,line width=2] {0.165*(x+0.6)^(-0.8)+0.045*exp(-40*x^(-1.3))}; 

\addplot [fill=red,color=red,mark=*,only marks,fill opacity=0.5,draw opacity=0.8, mark size=2.5,draw= black,clip mode=individual]
table{%			
0.8301	0.0246
1.8078	0.0154
15.1456	0.0590
4.0233	0.0261
6.5847	0.0556
22.0252	0.0603
138.7410	0.0834
43.3938	0.0679
1.3830	0.2228
3.5252	0.1914
15.8890	0.2120
6.8529	0.2476
2.1425	0.0458
5.6826	0.0426
22.0311	0.0349
8.4971	0.0326
3.2374	0.0289
8.0815	0.0238
44.4942	0.0393
16.1068	0.0323
3.2107	0.0409
8.4115	0.0371
40.5354	0.0469
14.8155	0.0394
1.9312	0.0307
5.4462	0.0323
25.4338	0.0384
8.1110	0.0245
24.5668	0.0402
9.0398	0.0341
4.0438	0.0567
9.4668	0.0410
42.1998	0.0445
16.7367	0.0439
4.3116	0.0644
9.5574	0.0418
39.6663	0.0393
17.7679	0.0495
3.5367	0.0521
31.5768	0.0300
12.9928	0.0318
2.9239	0.0298
31.0748	0.0242
12.0597	0.0229
1.8606	0.0341
5.3369	0.0371
30.8000	0.0673
11.5784	0.0597
1.7162	0.0349
4.8936	0.0375
25.3836	0.0550
10.1807	0.0556
2.9370	0.0250
34.5710	0.0250
16.6623	0.0364
};



\addplot [fill=black,color=black,mark=diamond*,only marks,fill opacity=0.5,draw opacity=0.8, mark size=3,draw= black,clip mode=individual]
table{%
1.1158	0.0594
1.1321	0.0464
1.4994	0.0694
0.5786	0.0564
1.6944	0.0789
1.7591	0.0765
1.1122	0.0867
1.0589	0.0712
1.1571	0.0876
1.2165	0.0676
1.2344	0.0819
1.2363	0.0877
1.3313	0.0823
1.3627	0.0883
1.4230	0.0847
1.5849	0.1090
1.7396	0.0983
1.5660	0.1047
1.8579	0.0524
1.9424	0.0833
1.8898	0.0935
1.8852	0.1147
1.7887	0.1142
1.2929	0.0762
1.3288	0.0760
1.2820	0.0661
0.8577	0.0852
0.8807	0.0819
1.0269	0.1856
0.9488	0.1445
2.0313	0.0845
1.9035	0.0891
1.9157	0.1012
1.1717	0.1009
1.1038	0.0912
1.2733	0.1250
1.3075	0.1444
1.2379	0.0814
1.4532	0.1142
1.4085	0.1106
1.4691	0.0997
1.5815	0.1103
1.6286	0.0989
1.4421	0.0625
1.6580	0.0629
1.6724	0.0525
1.7193	0.0867
1.7314	0.0735
1.7527	0.0878
1.1900	0.0700
1.3414	0.0742
1.4175	0.0828
1.2412	0.0828
1.4511	0.0802
1.5629	0.0887
1.2886	0.1100
1.2377	0.1326
};

\end{groupplot}
\end{tikzpicture}

==> tab1.tex <==
\renewcommand*{\arraystretch}{1}
\begin{center}
\begin{small}
\begin{table}[h!]
\centering
\caption{Shape factors $\beta_p = (A_\text{proj} D_p)/\mathcal{V}_p$ for selected plastic geometries; note that the diameters are calculated as sphere-volume equivalent diameter $D_p = \sqrt[3]{\frac{6}{\pi} \mathcal{V}_p}$}
\begin{tabular}{c c c c c c c c}
\toprule
\begin{tabular} {@{}c@{}}Shape/ \\ Parameter \end{tabular} & \begin{tabular} {@{}c@{}}Sphere \\ \phantom{P}  \end{tabular} & \begin{tabular} {@{}c@{}}Cylinder \\ \phantom{P} 
\end{tabular} &  \begin{tabular} {@{}c@{}}Cube \\\phantom{P}   \end{tabular} & \begin{tabular} {@{}c@{}}Rectangular prism \\ \phantom{P}  \end{tabular}\\
\midrule
$\mathcal{V}_p$ (m$^3$) &  $\frac{\pi D_p^3}{6}$ & $\frac{\pi D^2 a}{4}$ & $a^3$  & $abc$\\ 
$A_\text{proj}$ (m$^2$) &  $\frac{\pi D_p^2}{4}$ & $a D$ & $a^2$ & $bc$\\
$D_p$ (m) &  $D_p$ & $\sqrt[3]{1.5 D^2 a}$
&$\sqrt[3]{\frac{6}{\pi}}a$ &$\sqrt[3]{\frac{6}{\pi}  abc}$ \\
$\beta_p$ ($-$) & 1.5 & $4\sqrt[3]{1.5a}/(\pi D^{1/3})$ & 1.24 & $\sqrt[3]{\frac{6}{\pi} a b c}/a$\\
\multicolumn{5}{c}{
\hspace{1.7cm}
\begin{tikzpicture}
\draw (0,0) circle (0.75cm);
\draw (-0.75,0) arc (180:360:0.75 and 0.5);
\draw[dashed] (0.75,0) arc (0:180:0.75 and 0.5);
\fill[fill=black] (0,0) circle (1pt);
\draw[dashed] (-0.75,0) -- node[above]{$D_p$} (0.75,0);
\end{tikzpicture}
\hspace{0.1cm}
\begin{tikzpicture}
\draw (-0.75,0) arc (180:360:0.75 and 0.5);
\draw[dashed] (0.75,0) arc (0:180:0.75 and 0.5);
\draw (0.75,1.5) arc (0:360:0.75 and 0.5);
\fill[fill=black] (0,0) circle (1pt);
\draw[dashed] (-0.75,0) -- node[above]{$D$}(0.75,0);
\draw[solid] (0.75,0) -- node[right]{$a$}(0.75,1.5);
\draw[solid] (-.75,0) -- (-0.75,1.5);
\end{tikzpicture}
\hspace{0cm}
\begin{tikzpicture}
\draw (0,1,0) -- node[above]{$a$}(1,1,0) -- (1,0,0) -- (1,0,1) -- (0,0,1) -- (0,1,1) -- cycle;
\draw[line cap=round] (1,1,1) -- (0,1,1) (1,1,1) -- (1,0,1) (1,1,1) -- (1,1,0);
\draw[dashed] (0,0,0) -- (0,1,0);
\draw[dashed] (0,0,0) -- (0,0,1);
\draw[dashed] (0,0,0) -- (1,0,0);
\end{tikzpicture}
\hspace{0.2cm}
\begin{tikzpicture}
\draw (0,1.5,-1) -- node[above]{$a$}(1,1.5,-1) -- node[right]{$b$} (1,0,-1) -- node[right]{$c$}(1,0,1) -- (0,0,1) -- (0,1.5,1) -- cycle;
\draw[line cap=round] (1,1.5,1) -- (0,1.5,1) -- (1,1.5,1) -- (1,0,1) (1,1.5,1) -- (1,1.5,-1);
\draw[dashed] (0,0,-1) -- (0,1.5,-1);
\draw[dashed] (0,0,-1) -- (0,0,1);
\draw[dashed] (0,0,-1) -- (1,0,-1);
\end{tikzpicture}
}\\
\bottomrule
\end{tabular}
\label{table:conditions}
\end{table}
\end{small}
\end{center}




